Construction and Elicitation of a Black Box Model in the Game of Bridge

We address the problem of building a decision model for a specific bidding situation in the game of Bridge. We propose the following multi-step methodology i) Build a set of examples for the decision problem and use simulations to associate a decision to each example ii) Use supervised relational learning to build an accurate and readable model iii) Perform a joint analysis between domain experts and data scientists to improve the learning language, including the production by experts of a handmade model iv) Build a better, more readable and accurate model.

==> introEng.tex <==
% !TEX root =./mainEng.tex
% !TEX encoding = UTF-8 Unicode
\section{Introduction}
Our goal is to model expert decision processes in Bridge. To do so, we propose a methodology involving human experts, black box decision programs, and relational supervised machine learning systems. The aim is to obtain a global model  for this decision process, that is both expressive and has high  predictive performance. 


Following the success of supervised methods of the deep network family, and a growing pressure from society imposing that automated decision processes be made more transparent,
 a growing number of AI researchers are (re)exploring techniques to interpret, justify, or explain ``black box" classifiers (referred to as the Black Box Outcome Explanation Problem \cite{GuidottiMRTGP19}). It is a question of 
 building, a posteriori, explicit models in symbolic languages, most often in the form of rules or decision trees that explain the outcome of the classifier in a format intelligible to an expert. 
Such explicit models extracted by supervised learning can carry expert knowledge \cite{inter-ml}, which has intrinsic value for explainability, pedagogy, and evaluation in terms of ethics or equity (they can help to explain biases linked to the learning system or to the set of training examples).
%Learning a global model (i.e. capable of explaining the class of any example)  that is both interpretable and highly accurate has been identified as a difficult problem. Many recent approaches that build interpretable models adopt a simpler two-step method: a first step aims to build a global black box classifier that is as precise as possible, a second step focuses on the generation of a set of local explanations (linear models/rules) to justify the classification of a specific example (see for instance the popular LIME \cite{LIME} and ANCHORS \cite{ANCHORS} systems).
The vast majority of works focus on local interpretability of decision models: 
 simple local explanations (linear models/rules) are  built to justify individual predictions 
of black box classifiers (see for instance the popular LIME
\cite{LIME} and ANCHORS \cite{ANCHORS} systems).
 Such local explanations do not give an overview of the black box model behaviour, 
they moreover rely of the notion of neighborhood of instances to build explainations and may be highly unstable.   
Our approach is to build post-hoc global explanations by approximating the predictions of black box models with 
 interpretable models such as decision lists and rule sets.
%The black box classifier can also be used to generate, on demand, additional examples to better target the explanations \cite{abs-1805-10820}.
 %A counterfactual explanation of a prediction describes the smallest change to the feature values that changes the prediction to a predefined output. Counterfactual explanations are also a very promising technique for extracting a factual/local explanation for a complex decision problem \cite{molnar2019}.
 
 We present here a complete methodology for acquiring a global model of a black box classifier as a set of relational rules, both as explicit and as accurate as possible. As we consider a game, i.e. a universe with precise and known rules, we are in the favorable  case where it is possible to generate, on demand, data that i)  is in agreement with the problem specification, and ii) can be labelled with correct decisions through simulations.    The methodology we propose consists of the following elements:
 \begin{enumerate}
 \item Problem modelling with relational representations, data generation and labelling.
 \item Initial investigation of the learning task and learning with relational learners.
 \item Interaction with domain experts  who refine a  learned model to produce a simpler  alternative model, which is more easily understandable for domain users.
 \item Subsequent investigation of the learning task, taking into account the concepts used by experts to produce their  alternative model, and the proposition of a new, more accurate model.
  \end{enumerate}
 The general idea is to maximally leverage interactions between experts and engineers, with each group building on the analysis of the other. 
 
 
 We approach the  learning task using relational supervised learning methods from \emph{Inductive Logic Programming} (ILP)   \cite{MuggletonR94}.  The language of these methods, a restriction of first-order logic, allows learning compact rules, understandable by experts in the domain.  The logical framework   allows   the use of a domain vocabulary together with domain knowledge defined in a domain theory, as illustrated in early work on the subject \cite{ilpbridgegamechallenge}.  
 
 The outline of the article is as follows. After a brief introduction to bridge in Section \ref{13bridgepb}, we describe in Section \ref{13genedonnees} the relational formulation of the target learning problem, and the method for generating and labelling examples.
 We then briefly describe in Section \ref{13ilp} the ILP systems used, and the first set of experiments run on the target problem, along with their results (Section \ref{13expes}). In Section \ref{13analyse}, bridge experts review a learned model's output and build a powerful  alternative model of their own, an analysis of which leads to a refinement of the ILP setup and further model improvements. Future research avenues are outlined in the conclusion.

==> plot/egc2020-ENG-arXiv/apprentissageENG.tex <==
\section{Learning Expert Rules by Inductive Logic Programming}
\label{ilp}
\subsection{ Inductive Logic Programming Systems}
The ILP systems used in our experiments were \emph{Aleph} and \emph{Tilde}. These are two state of the art ILP systems, quite different in their learning strategy. 
\subsubsection{Aleph}
Aleph \cite{aleph} learns by entailment \cite{MuggletonR94}: given a set of positive examples $E^+$, a set of negative examples $E^-$, each as ground literals of the target concept predicate and a domain theory $T$, the goal of learning by entailment is to find a \emph{hypothesis} $H$  as a logic program, i.e. a set of definite clauses, such that $\forall e^+ \in E^+: H \wedge T \models e^+$ and $\forall e^- \in E^- : H \wedge T \not \models e^-$. In other words, given the domain theory $T$, and after learning hypothesis $H$, it is possible  from each positive example description $e^+$ to derive that $e^+$ is indeed a positive example, while such a derivation is impossible for any of the negative examples $e^-$.  
%It is required that the truth of positive examples is a consequence of $H$ and $T$, while the truth of negative examples is not. 
Positive examples are then said to be \emph{covered} by $T$ and $H$. The domain theory $T$ is represented by a set of facts, i.e. ground positive literals from other predicates and clauses.  $H$ is a set of definite clauses where the head predicate of each rule is the target predicate.  An example of  such a hypothesis $H$ is given in Listing \ref{best-rules-aleph}.


In our problem, the target predicate is \emph{decision}, as defined in Section \ref{targetPredicate}.  When the example is positive,  the literal is as exemplified in Section \ref{targetPredicate}, whereas, when the example is negative,  the last argument \emph{bid} is replaced with \emph{pass}. Under this framework, we look for a logic program that entails examples with the bid argument, and does not entail examples with the pass argument.   The domain theory is represented by ground literals from other predicates   together with definite clauses that  enrich the representation of the examples (see Section \ref{modrel}).
% Part of this domain theory has already been used in another application of these same  ILP  systems for decision making in a bidding problem \cite{ilpbridgegamechallenge}, which illustrates the reusability of this domain theory.   

The  Aleph standard strategy \emph{induce} learns the logic program as a set of rules  using a hedging strategy: First, it selects a  seed positive example $e$ not entailed  by the current solution. Then, it performs a top-down search in a space  whose lower bound is a maximally specific clause (denoted $B$) constructed from the  seed $e$ and the domain theory.  %Aleph traverses the generalization space of $B$ satisfying the expert user-defined language bias. 
Once a rule $R_e$ is learned for $e$, the positive examples covered by $R_e$ are removed from the learning set, and learning resumes on this new set until all positive examples are covered. Since this strategy requires a seed to be chosen, it is sensitive to the order of the learning examples.
%when the default path strategy (\texttt{best\_first}) is used. 
We also used Aleph with \emph{induce\_max}, which is insensitive to the order of positive examples, but is a more expensive search strategy. It constructs a single coverage of all positive examples by choosing the best clause (in terms of coverage) covering each positive example. This gives the resulting clauses a large overlap, which has proved beneficial in some of our experiments. 
\subsubsection{Tilde}
Tilde\footnotemark \cite{Blockeel:1998aa} relies on the
% from interpretations, more restricted than learning by implication but sufficient for learning in the field of bridge. \cite{ilpbridgegamechallenge} 
%. Given a set of classes $C$=\{ $c_i$\} (represented by predicates without arguments), a set of $E$ examples described as interpretations, i.e. as sets of facts, associated with a class and a $B$ domain theory in the form of clauses, the goal is to construct a hypothesis $H$ (a decision tree, which can be translated into a logical program), such as $\forall (e, c) \in E, H \wedge e \wedge B \models c$, and $\forall c' \in C - c: Hedge and B models c$.
\emph{learning by interpretation} setting.
\footnotetext{Available as part of the ACE Ilp system at \url{https://dtai.cs.kuleuven.be/ACE/}}
This setting is more restrictive than learning by implication, but is sufficient for learning rules in the field of Bridge: the interpretation domain is finite, and the problem addressed does not require, a priori, the learning of recursive rules.  
%\begin{quote}
%\textit{Since in learning from interpretations, the class of an example is assumed to be independent of other examples, 
%this setting is less powerful than the standard ILP setting (e.g., for what concerns recursion). With this loss of power comes %a gain in efficiency, through local coverage tests. 
%The interesting point is that the full power of standard ILP is not used for most practical applications, and learning 
%from interpretations usually turns out to be sufficient for %practical applications.}
%\end{quote}
%This is the case for our classification problem.
%; we are more interested here in benchmarking these systems, and in the different models they compute. 
Tilde learns  a relational binary decision tree in which the nodes  are conjunctions of literals that can share variables  with the following restriction: a variable introduced in a node cannot appear in the right branch below that node (i.e. the failure branch of the test associated to the node). In the decision tree, each example, described through a set of ground literals,  is propagated through the current tree until it reaches a leaf. In the final tree, each leaf is associated to the decision \emph{bid}/\emph{pass}, or a probability distribution on these decisions.  An example of a Tilde decision tree output is given in Listing \ref{best-tree-tilde}.

 %The need for this restriction follows from the semantics of the tree. 
 %A variable $X$ that is introduced in a node is quantified existentially within the conjunction of that node. 
 %The right subtree is only relevant when the conjunction fails ("there is n Translated with www.DeepL.com/Translator (free version)
%
%
%\section{Apprentissage de règles expertes à l'aide de systèmes de  ILP }
%\label{ilp}
%\subsection{Les systèmes choisis}
%Les systèmes de  ILP  \cite{MuggletonR94} que nous avons utilisés dans nos expériences sont Aleph \cite{aleph} et Tilde \cite{tilde}. Ce sont deux systèmes de  ILP  de l'état de l'art, assez différents dans leur stratégie d'apprentissage. 
%
%Aleph apprend par implication  (\textit{learning from entailment}) \cite{MuggletonR94}. \'Etant donné un ensemble d'exemples positifs $E^+$, un ensemble d'exemples négatifs $E^-$ et une théorie du domaine  $T$, le but de l'apprentissage est de trouver un programme logique (un ensemble de clauses) $H$, tel que  $\forall e \in E^+:  H \wedge T \models e$ et $\forall e \in E^- : H \wedge  T \not \models e$.
%Pour Aleph, les exemples sont des littéraux représentant la classe ($bid/1$). La théorie du domaine est représentée par un ensemble de faits et de règles qui vont permettre d'enrichir la représentation des exemples (voir Section \ref{modrel}). Une partie de cette théorie du domaine a déjà été utilisée dans une autre application de ces mêmes sys\-tè\-mes de  ILP  pour la prise de décision dans un problème d'enchères \cite{ilpbridgegamechallenge}, ce qui illustre bien la réutilisabilité de cette théorie du domaine.   
%Aleph dans sa version standard (\texttt{induce}) apprend des règles en utilisant une stratégie de couverture :  il sélectionne un exemple graine $e$ non couvert par la théorie courante.  Il parcourt ensuite de façon descendante un espace de recherche dont la borne inférieure est une clause maximalement spécifique (notée $B$) construite à partir de la graine $e$ et de la théorie du domaine.  %Aleph  parcourt l'espace des généralisations de $B$ satisfaisant le biais de langage défini par l'utilisateur expert. 
%Une fois une règle $R_e$ apprise pour $e$, les exemples positifs couverts par $R_e$ sont effacés de l'ensemble d'apprentissage et l'apprentissage reprend sur ce  nouvel ensemble, jusqu'à ce que tous les exemples positifs soient couverts. A cause du choix de la graine $e$, Aleph est sensible à l'ordre des exemples d'apprentissage lorsque la stratégie de parcours par défaut (\texttt{best\_first}) est utilisée. 
%Nous avons également utilisé  Aleph avec une stratégie plus coûteuse (\texttt{induce\_max})  insensible à l'ordre des exemples positifs. Elle construit une unique couverture de l'ensemble des exemples positifs en choisissant la meilleure clause (en terme de couverture) couvrant chaque exemple positif. Les clauses obtenues ont alors  un recouvrement important, ce qui s'est avéré bénéfique dans nos expériences.
%
%Tilde apprend un arbre de décision relationnel
%% à partir d'interprétations, plus restreint que l'apprentissage par implication  mais suffisant pour l'apprentissage dans le domaine du bridge. \cite{ilpbridgegamechallenge} 
%%. Etant donné un ensemble de classes $C$=\{ $c_i$\} (représentées par des prédicats sans arguments), un ensemble d'exemples $E$ décrits comme des interprétations, c'est à dire comme des ensembles de faits, associés à une classe et une théorie du domaine $B$  sous forme de clauses, le but est de construire une hypothèse $H$ (un arbre de décision, qui peut se traduite sous forme d'un programme logique), tel que $\forall (e, c) \in E,  H \wedge e \wedge B \models c$, and $\forall c' \in C  - c: H \wedge e \wedge B \not \models c'$.
%%Ce cadre d'apprntissage par interprétations est plus restreint que l'apprentissage par implication \cite{tilde} mais est suffisant pour l'apprentissage de règles dans le domaine du bridge : le domaine de l'interprétation est fini, et le problème adressé ne nécessite pas, \textit{a priori}, d'apprendre des concepts récursifs.  
%%\begin{quote}
%%\textit{Since in learning from interpretations, the class of an example is assumed to be independent of other examples, 
%%this setting is less powerful than the standard ILP setting (e.g., for what concerns recursion). With this loss of power comes %a gain in efficiency, through local coverage tests. 
%%The interesting point is that the full power of standard ILP is not used for most practical applications, and learning 
%%from interpretations usually turns out to be sufficient for %practical applications.}
%%\end{quote}
%%This is the case for our classification problem.
%%;  we are more interested here in benchmarking these systems, and in the different models they compute. 
% c'est-à-dire  un arbre de décision binaire  dans lequel les sommets de l'arbre sont des conjonctions de littéraux pouvant partager des variables, avec la restriction suivante : une  variable introduite dans un sommet  ne peut pas apparaître dans la branche droite  sous ce sommet (la branche d'échec du test porté par le sommet). 
% %The need for this restriction follows from the semantics of the tree. 
% %A variable $X$ that is introduced in a node is quantified existentially within the conjunction of that node. 
% %The right subtree is only relevant when the conjunction fails (“there is no such $X$”), in which case further reference to 
% %$X$ is meaningless.
%Afin de spécialiser un sommet de requête associée $Q$, Tilde calcule une spécialisation de  $Q$ étant donné le biais de langage défini par l'utilisateur  et choisit la spécialisation qui maximise un critère de qualité, par défaut le gain d'information adapté au cas relationnel. 
%
%
%%The ILP systems allow for using a powerful and flexible target representation language  through the use of explicit 
%%background knowledge, here represented as a set of definite clauses. To cope with the increased size of the hypothesis space, 
%%both Aleph and Tilde allow the user to define the search space through sophisticated \textit{language bias}. This language 
%%bias can be seen as a grammar-like user defined specification of the search space.  
%
%\subsection{Paramétrage d'Aleph et Tilde}
%
%Nous abordons ici les différents choix de paramètres retenus pour Aleph et Tilde pour l'expérience présentée dans la Section suivante. Certains de ces choix sont inhérents à l'algorithme utilisé, d'autres ont été réalisés pour des raisons de performances, de lisibilité du modèle induit ou par souci de simplicité d'implémentation. Nous ne présentons que les paramétrages les plus significatifs pour chaque système \cite{aleph,tildeuserguide}.
%
%\paragraph{Biais de langage}
%Le biais de langage spécifie pour les deux algorithmes de  ILP  l'espace de recherche, en décrivant quels prédicats vont former les hypothèses, et quels arguments peuvent prendre ces prédicats : pour chaque prédicat d'arité non nulle, on peut préciser la nature de ses arguments (variable ou constante, entrée ou sortie \footnote{Une variable en entrée apparaît dans la partie gauche de la clause en construction, alors qu'une variable de sortie n'apparaît pas encore dans la clause courante et est donc existentiellement quantifiée.}).
%De plus, Aleph peut manipuler des termes complexes. Il peut ainsi au cours de sa recherche construire une clause dont un des termes est une liste partiellement instanciée : $distribution(A,[B,C,2,1]) $ dénote une distribution d'une main dont les  deux couleurs les plus courtes sont 2 et 1,  les longueurs des deux couleurs les plus longues étant  non spécifiées.  
%La fonctionnalité \texttt{lookahead} de Tilde lui permet de créer des noeuds testant une conjonction de littéraux. L'usage de $nb(E,Suit,Value)$, et de $gteq$ ou $lteq$ lui permet  de décrire la longueur d'une couleur spécifique ou non et d'ainsi généraliser la notion de distribution en effectuant de multiple tests sur les différentes couleurs. %Aleph ne manipule pas aussi bien ce genre d'abstraction, qui requiert de construire des clauses de taille plus longue.
%
%Certains biais de langage ont aussi été introduits en concertation avec les experts du domaine, après des expériences d'apprentissage préliminaires. Par exemple, ils n'étaient pas satisfaits de certains prédicats apparaissant dans les hypothèses trop spécifiques autour d'une notion qu'ils estimaient présentant une symétrie. Après rectification, les modèles construits ne faisaient plus intervenir cette notion, sans perte de précision sur les ensembles de tests, validant \textit{a posteriori} le biais de langage choisi.
%
%\paragraph{Options de recherche}
%
%Nous avons choisi les options de recherche des algorithmes par défaut quand cela était possible pour Aleph et Tilde. Les paramètres de Tilde sont exclusivement ceux par défaut. Pour Aleph : \textit{clauselength}=6 (la longueur maximum de la règle générée), \textit{minpos}=5 (le nombre minimum d'exemples positifs couverts par la régle) , \textit{minacc} = 0.85 et \textit{noise}= inf (le nombre maximum d'exemples négatifs couverts par une règle); pour Tilde : \textit{heuristic} = gainratio, \textit{pruning} = c45 safe pruning, \textit{stopping criterion}  = mincase.


==> plot/egc2020-ENG-arXiv/conclusionENG.tex <==
\section{Conclusion}
\label{conclusion}
We conducted  an end-to-end experiment to acquire expert rules for a bridge bidding problem. 
%The results obtained validate our working hypotheses. 
We did not propose  new technical tools, our contribution was in investigating a complete methodology to handle a learning task from beginning to end, i.e.  from the specifications of the learning problem to a learned model,  obtained after expert feedback, who not only criticise and evaluate the models, but also propose hand-made (and computable)  alternative models. The methodology includes generating and labelling  examples by using both domain experts (to drive the modelling and relational representation of the examples) and a powerful simulation-based black box  for labelling. The result is a set of high quality examples, which is a prerequisite for learning a compact and accurate  relational model. The final relational model is built after an additional phase of interactions with experts, who investigate  a learned model, and propose an alternative model, an analysis of which leads to further refinements of the learning language. We argue that  interactions between experts and engineers are made easy when the learned models are relational, allowing experts to revisit and contradict  them.

Clearly, learning tasks in a well defined and simple universe with precise and deterministic  rules, such as in games,  are good candidates for the interactive methodology we proposed. The extent to which experts and learned models cooperating in this way can be transferred to less well defined problems, including, for instance, noisy environments, has yet to be investigated. Note that complementary techniques can also be applied, such as active learning, where machines or humans dynamically provide  new examples to the system, leading to revised models. Overall, our contribution is a step towards a complete handling of learning tasks for decision problems, giving domain experts (and non-domain experts alike) the tools to both make accurate decisions, and to understand and scrutinize the logic behind those decisions.

%Last sentence of old conclusion
%. Overall, our contribution is a step towards a complete handling of learning tasks for decision problems, from start to end products agreed at least by domain experts and as much as possible to the non experts who in fine have to take decisions

==> plot/egc2020-ENG-arXiv/jpENG.tex <==
\section{Problem Addressed}
\label{bridgepb}
\subsection{Brief Introduction to the Game of Bridge} 

Bridge is played by four players in two competing partnerships, namely, \emph{North} and \emph{South} against \emph{East} and \emph{West}. A classic deck of 52 playing cards is shuffled and then dealt evenly amongst the players ($\frac{52}{4}=13$ cards each). The objective of each side is to maximize a score which depends on:
\begin{itemize}
    \item \textbf{The vulnerability} of each side. A \emph{non-vulnerable} side loses a low score when it does not make it's contract, but earns a low score when it does make it. In contrast, a \emph{vulnerable} side has higher risk and reward.
    \item \textbf{The contract} reached at the conclusion of the \emph{auction} (the first phase of the game). The contract is the commitment of a side to win a minimum of $l_{min} \in \{7, \dots 13\}$ tricks in the \emph{playing phase} (the second phase of the game). The contract can either be in a \emph{Trump} suit (\Cs{}, \Ds{}, \Hs{}, \Ss{}), or \emph{No Trumps} (\NT{}), affecting which suit (if any) is to gain extra privileges in the playing phase. An opponent may \emph{Double} a contract, thus imposing a bigger penalty for failing to make the contract (but also a bigger reward for making it). A contract is denoted by $pS$ (or $pS^X$ if it is Doubled), where $p=l_{min} - 6\in \{1, \dots 7\}$ is the \emph{level} of the contract, and $S \in \{\Cs{},\Ds{},\Hs{},\Ss{},NT\}$ the \emph{trump suit}. The holder of the contract is called the \emph{declarer}, and the partner of the declarer is called the \emph{dummy}.
    \item \textbf{The number of tricks won} by the declaring side during the playing phase. A trick containing a trump card is won by the hand playing the highest trump, whereas a trick not containing a trump card is won by the hand playing the highest card of the suit led.
\end{itemize}
\bigskip
 For more details about the game of bridge, the reader can consult \cite{acbl}. Two concepts are essential for the work presented here:
\begin{itemize}
\item {\bf Auction}: This allows each player (the first being called the \emph{dealer}) the opportunity to disclose coded information about their hand or game plan to their partner\footnotemark. Each player bids in turn, clockwise, using as a language the elements: \emph{Pass}, \emph{Double}, or a contract higher than the previous bid (where $\Cs{} < \Ds{} < \Hs{} < \Ss{} < NT$ at each level). The last bid contract, followed by three Passes, is the one that must be played.

\item {\bf The evaluation of the strength of a hand}: Bridge players assign a value for the highest cards: an Ace is worth 4\,HCP (\emph{High Card Points}), a King 3\,HCP, a Queen 2\,HCP and a Jack 1\,HCP. Information given by the players in the auction often relate to their number of HCP and their \emph{distribution} (the number of cards in one or more suits).

\end{itemize}
\footnotetext{The coded information given by a player is decipherable by both their partner and the opponents, so one can only deceive their opponents if they're also willing to deceive their partner. In practice, extreme deception in the auction is rare, but for both strategical and practical reasons, the information shared in the auction is usually far from complete.}


\subsection{Problem Statement} 

After receiving suggestions from bridge experts, we chose to analyse the following situation:
\begin{itemize}
\item West, the dealer, bids \Ss{4}, which (roughly) means that they have a minimum of 7 spades, and a maximum of 10\,HCP in their hand.
\item North Doubles, (roughly) meaning that they have a minimum of 13\,HCP and, unless they have a very strong hand, a minimum of three cards in each of the other suits (\Cs{}, \Ds{} and \Hs{}).
\item East passes, which has no particular meaning.
\end{itemize}
South must then make a decision: pass and let the opponents play $4\Ss{}^X$, or bid, and have their side play a contract. This is a high stakes decision that bridge experts are yet to agree on a precise formulation for. Our objective is to develop a methodology for representing this problem, and to find accurate and explainable solutions using relational learners. It should be noted that Derek Patterson was interested in solving this problem using genetic algorithms \cite{patterson}.


In the remainder of the article, we describe the various processes used in data generation, labelling, supervised learning, followed by a discussion of the results and the explicit models produced. These processes use relational representations of the objects and models involved, keeping bridge experts in the loop and allowing them to make adjustments where required.

In the next section we consider the relational formulation of the problem, and the data generation and labelling.


\section{Automatic Data Generation Methodology}
\label{genedonnees}
%\subsection{General Overview}
The methodology to generate and label the data consists of the following steps:
\begin{itemize}
\item Problem modelling
\item Automatic data generation
\item Automatic data labelling 
\item ILP framing
\end{itemize}
These steps are the precursors to running relational rule induction (Aleph) and decision tree induction (Tilde) on the problem.
\subsection{Problem Modelling} \label{problemModelling}
The problem modelling begins by asking experts to define, in the context described above, two rule based models: one to characterize the hands such that West makes the \Ss{4} bid, and another to characterize the hands such that North makes the Double bid.  These rule based models are submitted to simulations allowing the experts to interactively validate their models. With the final specifications, we are able to generate examples for the target problem. For this section we introduce the terms:
\begin{itemize}
    \item \emph{nmpq exact distribution} which indicates that the hand has $n$ cards in \Ss{}, $m$ cards in \Hs{}, $p$ cards in \Ds{} and $q$ cards in \Cs{}, where $n+m+p+q=13$.
    \item \emph{nmpq distribution} refers to an exact distribution sorted in decreasing order (thus ignoring the suit information). For instance, a $2533$ exact distribution is associated to a $5332$ distribution.
    \item $|c|$ is the number of cards held in the suit $c\in\{\Ss{},\Hs{},\Ds{},\Cs{}\}$.
\end{itemize}

\subsubsection{Modelling the 4\Ss{} bid} \label{fsBid}
Experts have modeled the 4\Ss{} bid by defining a disjunction of 17 rules that relate to West hand:
\begin{equation} \label{fsRules}
4\Ss{} \leftarrow \bigvee\limits_{i=1}^{17} R_i, \mbox{ where } R_i = C_0 \wedge V_i \wedge C_i 
  \end{equation}
  in which 
\begin{itemize}
    \item $C_0$ is a condition common to the 17 rules and is reported in Listing \ref{common-4s-rules} in the Appendix.
    \item $V_i$ is one of the four possible vulnerability configurations (no side vulnerable, both sides vulnerable, exactly one of the two sides vulnerable).
    \item $C_i$ is a condition specific to the $R_i$ rule.
\end{itemize}
For instance, the conditions for rules $R_2$ and $R_5$ are:
\begin{itemize}
	\item $V_2=$ East-West not vulnerable, North-South vulnerable.
	\item $C_2=$ all of: 
	\begin{itemize}
        \item $|\Hs{}|=1$,
       	\item  2 cards exactly among Ace, King, Queen and Jack of \Ss{}, 
        \item a 7321 distribution.
    \end{itemize}
	\item $V_5=$ East-West not vulnerable, North-South vulnerable.
	\item $C_5=$ all of: 
	\begin{itemize}
		\item $|\Cs{}| \geq 4$ or $|\Ds{}| \geq 4$, 
	    \item 2 cards exactly among Ace, King, Queen and Jack of \Ss{},  
	    \item a $7mpq$ distribution with $m\geq4$.
    \end{itemize}
\end{itemize}
To generate boards that satisfy these rules, we randomly generated complete boards (all 4 hands), and kept the boards where the West hand satisfies one of the 17 rules.
The experts were able to iteratively adjust the rules as they analysed the boards that passed through the filter.
After the experts were happy with the samples, 8,200,000 boards were randomly generated to analyse rule adherence, and 10,105 of them contained a West hand satisfying one of the 17 rules. All rules were satisfied at least once. $R_2$, for example, was satisfied 16.2\% of the time, and $R_5$ was satisfied 15\% of the time. 

\subsubsection{Double Modelling}
Likewise, the bridge experts also modeled the North Double by defining a disjunction of 3 rules relating to the North hand:
\begin{equation} \label{doubleRules}
\mbox{Double} \leftarrow \bigvee\limits_{i=1}^{3} R'_i, \mbox{ where }R'_i = C'_0 \wedge C'_i
\end{equation} 
This time, the conditions do not depend on the vulnerability.  The common condition $C'_0$ and the specific conditions $C'_i$ are as follows:
 \begin{itemize}
    \item $C'_0$ - for all $c, c_1, c_2\in\{\Hs{},\Ds{},\Cs{}\}$, $|c| \leq 5$ and not ($|c_1| = 5$ and $|c_2| = 5$).
    \item $C'_1$ - HCP $\geq$ 13 and $|\Ss{}| \leq$ 1.
    \item $C'_2$ - HCP $\geq$ 16 and $|\Ss{}| = 2$ and $|\Hs{}| \geq$ 3 and $|\Ds{}| \geq$ 3 and $|\Cs{}| \geq$ 3.
    \item $C'_3$ - HCP $\geq$ 20.
\end{itemize}
The same expert validation process was carried out as in Section \ref{fsBid}. A generation of 70,000,000 boards resulted in 10,007 boards being satisfied by at least one 4\Ss{} bid rule for the West hand and at least one Double rule for the North hand. All rules relating to Double were satisfied at least once. $R'_1$, for example. was satisfied 69.3\% of the time, and $R'_2$ was satisfied 24.8\% of the time.  

%\subsection{Automatic Data Generation}
%\label{genedonnees}
\subsection{Data Generation}\label{datageneration}
The first step of the data generation process is to generate a number of South hands in the context described by the 4\Ss{} and Double rules mentioned above. Note, again, that East's Pass is not governed by any rules, which is close to the real situation.

We first generated 1,000 boards whose West hands satisfied at least one \Ss{4} bid rule and whose North hands satisfied at least one  Double rule. One such board is displayed in Example \ref{example1}:
\begin{ex}
\label{example1}
 A board (North-South vulnerable / East-West not vulnerable)  which contains a  West hand satisfying rules $R_0$ and $R_5$ and a North hand satisfying rules $R'_0$ and $R'_1$:
{\footnotesize 
\begin{center}
\begin{bridgetable}

\begin{est}
\pique{10&3}
\coeur{J&8&4}
\carreau{A&7}
\trefle{Q&J&8&7&6&2}
\end{est}

\begin{ouest}
\pique{A&K&J&8&7&5&2}
\coeur{7}
\carreau{J&8&6&3}
\trefle{5}
\end{ouest}

\begin{sud}
\pique{Q&9&4}
\coeur{K&10&6&5&2}
\carreau{9&5}
\trefle{K&10&3}
\end{sud}

\begin{nord}
\pique{6}
\coeur{A&Q&9&3}
\carreau{K&Q&10&4&2}
\trefle{A&9&4}
\end{nord}

\end{bridgetable}
\end{center}
}
\end{ex}

For reasons that become apparent in Section \ref{dataLabel}, for each of the 1000 generated boards, we generate an additional 999 boards. We do this by fixing the South hand in each board, and randomly redistributing the cards of the other players until we find a board satisfying Equations \ref{fsRules} and \ref{doubleRules}. 
% The average calculation time is about  40" (with maximum calculation time: 10-15').
As a result of this process, 1,000  files are  created, with each file containing 1,000 boards that have the same South hand, but different West, North and East Hands. All boards satisfy Equations \ref{fsRules} and \ref{doubleRules}. 
\begin{ex}
\label{example2}
One of the 999 other boards generated:
\begin{itemize}
\item West hand: \Ss{}AK108653 \Hs{}4 \Ds{}832 \Cs{}84 
\item North hand: \Ss{}J2 \Hs{}AJ73 \Ds{}AK106 \Cs{}AJ9 
\item East hand: \Ss{}7 \Hs{}Q98 \Ds{}QJ74 \Cs{}Q7652 
\item  South hand: \Ss{}Q94 \Hs{}K10652 \Ds{}95 \Cs{}K103. 
\end{itemize}
Note that the South hand  is identical to the one in Example \ref{example1}, the West hand satisfies rules $R_0$ and $R_2$, and the North hand satisfies rules $R'_0$ and $R'_2$.
\end{ex}

\subsection{Data Labelling} \label{dataLabel}

The goal is to label each of the 1,000 South hands associated to the 1,000 sample files, with one of following labels:
\begin{itemize}
\item \textbf{Pass} when the best decision of South is to pass (and therefore have West play 4\Ss{}$^X$).
\item \textbf{Bid} when the best decision of South is to bid (and therefore play a contract on their side).
\item \textbf{?} when the best decision is not possible to be determined. We exclude these examples from ILP experiments.
\end{itemize}

Having bridge experts label a large number of these decisions would be difficult and costly, so we proceeded to label them computationally using the two following steps:
\begin{itemize}
\item Computing declarer's score by simulation.
\item Assigning labels.
\end{itemize}

\subsubsection{Scores Computation} 
During the playing phase, each player sees his own hand, and that of the dummy (which is laid face up on the table). A \emph{Double Dummy Solver} (DDS) is a computation (and a software) that calculates, in a deterministic way, how many tricks would be won by the declarer, under the pretext that everyone can see each other's cards. Though unrealistic, it is nevertheless a good estimator of the real distribution of tricks amongst the two sides \cite{pavlicek8J45}. For any particular board, a DDS can be run for all possible contracts, so one can thus deduce which contract will likely yield the highest score.

For each example file (which each contain 1,000 boards with the same South hand), a DDS software \cite{ddsrepo} was used to determine the score for the following situations:
\begin{itemize}
    \item 4\Ss{}$^X$ played by the East/West side.
    \item All available contracts played by the North/South side, with the exclusion of 4NT, 5NT, 5\Ss{}, 6\Ss{} and 7\Ss{} (experts deemed these contracts infeasible to be reached in practice). 
\end{itemize}

\subsubsection{Labels Allocation} The labels are assigned to a South hand  in the following way.
\begin{itemize}
    \item \textbf{Pass} in two cases:
    \begin{itemize}
        \item When South scores (on average) a better score by playing as a defender in the 4\Ss{}$^X$ contract than by bidding, even assuming that bidding will lead the North/South side to the best contract (best trump suit, best level), which is not guaranteed in practice.% in convenient.
        \item When South scores (on average) a significantly better score (30 points more) by playing as a defender in 4\Ss{}$^X$ than at any other available contract that North/South could play in themselves. 
      \end{itemize}
    \item \textbf{Bid} when there is an available contract in which South scores (on average) a better score than defending 4\Ss{}$^X$.
    \item \textbf{?} in other cases.
\end{itemize}

%\paragraph{Description statistique du jeu de données final} 
The initial dataset containing 1,000 sample files is reduced to a set $S$ of 960 examples after elimination of the 40 deals with the \emph{?} label. The resulting dataset consists of:
\begin{itemize}
    \item 338 \emph{Bid} labels, and
    \item 622 \emph{Pass} labels.
\end{itemize}


\subsection{Relational data modelling}
\label{modrel}
Now that we have generated and labeled our data, the next step is to create the relational representations to be used in relational learners. The learning task consists of using what is  known about a given board in the context described above, and the associated South hand, and predicting what the best bid is. The best bid is known for the labeled examples generated in the previous section, but, of course, unknown for new boards. 



We first introduce  the notations used in the remainder of the paper. 
\subsubsection{Logic Programming Notations}
\label{lp-notations}
Examples are represented by terms and relations between terms.  Terms are \textit{constants}  (for instance the integers between 1 and 13), or atoms whose identifiers start with a lower-case character (for instance \textit{west}, \textit{east}, \textit{spade}, \textit{heart}, \ldots) or \textit{variables}, denoted by an upper-case character ($X$, $Y$, $Suit$, \ldots). Variables may instantiate to any constant in the domain. Relations between objects are described using \textit{predicates} applied to terms. A \textit{literal} is a predicate symbol applied to terms, and a \textit{fact} is a  ground literal,  i.e. a literal without variables, whose arguments are ground terms only. For instance, \textit{decision([sq, s9, s4, hk, h10, h6, h5, h2, d9, d5, ck, c10, c3],4, n, west, bid)} is a ground literal of predicate symbol \textit{decision}, with four arguments, namely, a hand described as a list of cards,  and 4 constant arguments (see Section \ref{targetPredicate} for further details).
%We first present the chosen domain theory for  relational   learning algorithms. Most of the predicates used were introduced in \cite{ilpbridgegamechallenge}, among which $gteq(A, B)$ ($A\geq B$), $lteq(A, B)$ ($A \leq B$) or $nb(Hand, Suit, Number)$  (the suit $Suit$ of a hand $Hand$ has a length $Number$). For example, $nb(Hand,heart,3)$ means that the hand Hand contains 3  \Hs{} cards.

In order to introduce some flexibility in the problem description, the \textit{background knowledge} (also known as the \textit{domain theory})  is described as set of \textit{definite clauses}. We can think of a definite clause as a first order rule, containing a head (the conclusion of the rule) and a body (the conditions of the rule). For instance, the following clause: \\
$nb(Hand,Suit,Value) \leftarrow suit(Suit), count\_cards\_of\_suit(Hand,\allowbreak Suit, \allowbreak Value)$\\
has the head $nb(Hand,Suit,Value)$ where $Hand$, $Suit$ and $Value$ are variables  and two literals in the body  $suit(Suit)$  and  $count\_cards\_of\_suit(Hand,\allowbreak Suit,\allowbreak Value)$.
The declarative interpretation of the rule is that given that variable $Suit$ is a valid bridge suit, and given that $Value$ is the number of cards of the suit $Suit$ in the hand $Hand$, one can derive, in accordance with the logical consequence relationship $\models$ \cite{LLOYD-ILP} that $nb(Hand,Suit,Value)$ is true. 
This background knowledge will be used to derive additional information concerning the examples, such as hand and board properties. 

Let us now describe the \emph{decision} predicate, the target predicate of the relational learning task.

\subsubsection{Target Predicate}\label{targetPredicate} 
Given a hand, the position of the hand, vulnerability, and the dealer's position, the goal is to predict the class label. The target predicate for the bidding phase  is $\textit{decision}(Hand,\allowbreak Position,\allowbreak Vul,\allowbreak Dealer,\allowbreak Class)$ where the arguments are variables. 
\begin{itemize}
    \item $Hand$: the 13 cards of the player who must decide to \emph{bid} or \emph{pass}.
    \item $Position$: the relative position of the player to the dealer. In this task, Position is always 4, the South hand.
    \item $Vul$: the vulnerability configuration ($b$ = both sides,  $o$ = neither side, $n$ = North-South or $e$ = East-West).
    \item $Dealer$: the cardinal position of the dealer  among $north$, $east$, $south$ or $west$. In this task, Dealer is always $west$.
    \item $Class$: label to predict ($bid$ or $pass$).
\end{itemize}
In this representation, a labeled example is a grounded positive literal containing the decision predicate symbol.
% This footnote is no longer needed now that we have the lp notations section
%\footnotetext{A positive literal is a predicate such as $p(1,X)$, where $p$ is the predicate symbol. A grounded positive literal has no variables, e.g. $p(1,2)$. We do not use negative literals such as $\lnot p(X,Y)$ to describe hands and deals.}
% PARAGRAPHE N'EXISTANT PAS DANS LA VERSION COURTE EN FRANCAIS
Example 1 given in section \ref{datageneration} is therefore represented as: \\
$decision([sq,s9,s4,hk,h10,h6,h5,h2,d9,d5,ck,c10,c3],4,n,west,bid).$
% FIN PARAGRAPHE N'EXISTANT PAS DANS LA VERSION COURTE EN FRANCAIS
Such a ground literal contains all the explicit information about the example. However, in order to build an effective relational learning model of the target predicate as a set of rules, we need to introduce abstractions of this information, in the form of additional predicates in the domain theory. These predicates are described below.

\subsubsection{Target concept predicates} 


In order to learn a general and explainable model for the target concept, we need to carefully define the target concept representation language by choosing  predicate symbols that can appear in the model, more specifically, in the body of definite clauses for the target concept definition. We thus define new predicates in the domain theory, both extensional (defined by a set of ground facts) and intensional (defined by a set of rules or definite clauses). The updated domain theory allows to complete the example description, by gathering/deriving true facts related to the example. It also implicitly defines a target concept language that forms the search space for the target model which the Inductive Logic Programming algorithms will explore using different strategies. Part of the domain theory for this problem was previously used in another relational learning task for a bridge bidding problem \cite{ilpbridgegamechallenge}, illustrating the reusability of  domain theories.  The predicates in the target concept language are divided in two subsets:


\begin{itemize}
\item Predicates that were introduced in \cite{ilpbridgegamechallenge}. These include both general predicates, such as $gteq(A, B)$ ($A\geq B$), $lteq(A, B)$ ($A \leq B$) and predicates specific to bridge, such as $nb(Hand, Suit, Number)$, which tests that a suit $Suit$ of a hand $Hand$ has length $Number$ (e.g. $nb(Hand,heart,3)$ means that the hand $Hand$ has 3 cards in \Hs{})

\item Higher level predicates not used in \cite{ilpbridgegamechallenge}. Among which:
	\begin{itemize}
	\item $hcp(Hand,Number)$ is the number of High Card Points (HCP) in $Hand$.
	\item $suit\_representation(Hand,Suit,Honors,Number)$ is an  abstract representation of a suit.  $Honors$ is the list of cards strictly superior to 10 of the suit $Suit$ in hand $Hand$. $Number$  is the total number of cards in $Suit$ suit.
	\item $distribution(Hand, [N,M,P,Q])$ states that the $nmpq$ distribution (see Section \ref{problemModelling}) of hand $Hand$ is the ordered list $[N,M,P,Q]$. 

	\end{itemize}
\end{itemize}




% PARAGRAPHE N'EXISTANT PAS DANS LA VERSION COURTE EN FRANCAIS
For instance, in Example 1 from Section \ref{example1}, we  may add to the representation the following literals:
 \begin{itemize}
    \item $hcp([sq,s9,s4,hk,h10,h6,h5,h2,d9,d5,ck,c10,c3],8).$
    \item $suit\_representation([sq,s9,s4,hk,h10,h6,h5,h2,d9,d5,ck,c10,c3],spade,[q],3).$
    \item  $distribution([sq,s9,s4,hk,h10,h6,h5,h2,d9,d5,ck,c10,c3], [2,3,3,5]).$
\end{itemize}

Note again, that a fact (i.e. ground literal) can be independent of the rest of the domain theory, such as $has\_suit(hk,heart)$ which states that $hk$ is a  \Hs{} card, or it can be inferred from existing facts and clauses of the domain theory, such as
$nb([sq,s9,s4,hk,h10,h6,h5,h2,d9,d5,ck,c10,c3],heart,5)$, which derives from:
\begin{itemize}
\item $suit(heart)$:  $heart$ is a valid bridge suit.
\item $has\_suit(hk,heart)$: hk is a $heart$ card.
\item $nb(Handlist,Suit,Value) \leftarrow suit(Suit), count\_card\_of\_suit(Handlist,\allowbreak Suit,\allowbreak Value)$ where $count\_card\_of\_suit$  has a recursive definition   within the domain theory.
\end{itemize}
% FIN PARAGRAPHE N'EXISTANT PAS DANS LA VERSION COURTE EN FRANCAIS

%\subsubsection{Hand Representation} Bridge players abstract distributions into a partition of three classes: "$balanced$" hands (no suit of 0 or 1 card, one suit of 2 cards), "$semi\_balanced$" hands (no suit of 0 or 1 cards, exactly two suits of 2 cards) and "$unbalanced$" hands.

%Au bridge, 13 cartes suffisent à représenter entièrement une main. Cependant on peut grouper ces mains en familles partageant de propriétés communes.

%Le concept de distribution exacte par exemple, à savoir le nombre de carte par couleur est une métrique importante permettant d'évaluer le potentiel d'une main, au même titre que le compte des HCP présenté plus tôt.

%A titre d'exemple, la distribution exacte de la main de l'exemple 1 est 3-5-2-3 (3 \Ss{}, 5 \Hs{}, 2 \Ds{}, 3 \Cs{}).

%Cependant, un joueur de bridge raisonnera souvent en terme de motifs de mains dénotant la distribution des treize cartes parmi les quatre couleurs par ordre décroissant indépendamment de celles-ci ( e.g. 5-3-3-2 pour Exemple 1 ). Le terme distribution réfère par la suite à cette notion et non celle de distribution exacte.

%Cette notion peut être encore un peu plus abstraite en classant les mains de bridge parmi trois classes disjointes : $balanced$, $semi\_balanced$ et $unbalanced$ en fonction de leur distribution. Par exemple, les mains de la catégorie balanced sont les mains n'ayant aucune couleurs dites "courtes" (0 ou 1 carte) et au plus une couleur avec 2 cartes. 

%La règle suivante permet de saturer les exemples avec cette propriété : 
%\begin{verbatim}
%balanced(E) :- distribution(E,[4,3,3,3]).
%balanced(E) :- distribution(E,[4,4,3,2]).
%balanced(E) :- distribution(E,[5,3,3,2]).
%\end{verbatim}
%\comc{pareil}


==> plot/egc2020-ENG-arXiv/section56ENG2.tex <==
\subsection {First Experiments on  Relational Learning}
\label {expes}

Our first set of experiments applied the relational learners Aleph and Tilde to the relational representation presented in Section \ref{modrel}. For brevity, we call this representation the $L_0$ language in the experiments.  We first discuss the details of the experiment setup, followed be the results.
\subsection{Learning and evaluation setup}
The performance of the learning system with respect to  the size of the training set is averaged over $50$ executions $ i $. The sets $ Test_i $ and $ Train_i $ are built  as follows:
\begin {itemize}
	\item $Test_i = 140$ examples randomly selected from $S$ using seed $i$.
	\item Each $ Test_i $ is stratified, i.e. it has the same ratio of examples labeled $ bid $ as $ S $ (35.2 \%).
	\item $ Train_i = S \setminus Test_i $ (820 examples).
\end {itemize}

For each execution $ i $, we randomly generate from $Train_i$ a sequence of increasing number of examples $ n_k = 10 + 100 \times k $ with k between 0 and 8. We denote each of these subsets $ T_ {i, k} $, so that $|T_{i,k}|=n_k$ and $ T_ {i, k} \subset T_ {i, k + 1}$.
% The below is redundant, since the train set is shuffled randomly for each run anyway.
%The elements of each set $ T_ {i, k} $ are then randomly reordered (Aleph is sensitive to the ordering of the examples).
Each model trained on $ T_ {i, k} $ is evaluated on $ Test_i $. Figure \ref{accuracy_chart} presents the average accuracy (over all $ i = 1 \dots 50 $ executions) of the models trained on the sets $ T_ {i, k} $. The models are learned with Tilde and Aleph (with strategies \emph{induce} and \emph{induce\_max}). 

\subsection{Results}
% Old version before removing L0-aleph_induce
%As can be seen the chart (as well as in Table \ref{summary_table}), $L_0$-Aleph-induce had rather good accuracy with small models (in terms of the number of rules). After $310$ examples, the model size was stable at $\approx13$ rules. In contrast, the $L_0$-Tilde models had low accuracy, and a large number of nodes, which grew linearly with the number of training examples used. After an analysis of the Tilde output trees, it became apparent that Tilde was selecting many nodes with very specific conditions, in particular, with the \emph{suit\_representation} and \emph{distribution} predicates. While this improved performance in training, the specificity hindered the performance in testing.

Aleph failed to cope with the large $L_0$ language, and couldn't return a solution in reasonable time\footnotemark. As can be seen in Figure \ref{accuracy_chart} and Table \ref{summary_table}, the $L_0$-Tilde models had rather low accuracy and a large number of nodes (which grew linearly with the number of training examples used).

\footnotetext{Aleph was able to learn models after we removed the $nb$ predicate from $L_0$, albeit rather slowly ($\approx384$ core hours).
}

After an analysis of the Tilde output trees, it became apparent that Tilde was selecting many nodes with very specific conditions, in particular, with the \emph{suit\_representation} and \emph{distribution} predicates. While this improved performance in training, the specificity hindered the performance in testing. To counter this, we removed from $L_0$ the \emph{suit\_representation} and \emph{distribution} predicates, creating the more concise language $L_1$.

As expected, the average number of nodes in $L_1$-Tilde reduced dramatically. $L_1$-Tilde had the best accuracy of all models, which continued to increase between $610$ and $810$ examples. It's complexity was relatively stable, increasing only slightly between $510$ and $810$ examples, to a total of $21$ tree nodes.
% Note that the $L_1$-Tilde trees could have been found in $L_0$-Tilde (since $L_1$ is a subset of $L_1$), but since there was no punishment for creating extra nodes with \emph{suit\_representation} and \emph{distribution} to handle specific examples in the training set, those nodes dominated the tree.
%Comparing $L_0$-Aleph-induce results to   $L_1$-Tilde results 
With the smaller $L_1$ language, $L_1$-Aleph-induce was able to find solutions in reasonable time. It's accuracy was worse than that of $L_1$-Tilde ($85.6\%$ compared to $89.8\%$ when training on $810$ examples). After $310$ examples, the $L_1$-Aleph-induce model size remained stable at $16$ rules (it's accuracy also showed stability over the same training set sizes).

We were also able to use Aleph's \emph{induce\_max} strategy with $L_1$. Compared to \emph{induce}, this search strategy has a higher time cost and can produce rules with large overlaps in coverage, but can generalize better due to the fact that it saturates every example in the training set, not just a subset based on the coverage of a single seed example. This search strategy was of no benefit in this case, with $L_1$-Aleph-induce\_max showing slightly worse accuracy ($84.4\%$ compared to $85.6\%$) and a much higher complexity ($47$ rules compared to $15$) when compared with $L_1$-Aleph-induce.
%but the complexity remained quite low -- stabilizing at $\approx16$ rules. posted an average accuracy of $L_0$-Aleph-induce had rather good accuracy with small models (in terms of the number of rules). After $310$ examples, the model size was stable at $\approx13$ rulesIt's transition to $L_1$ caused almost no change in accuracy, while the model size stabilized at $\approx17$ rules (4 more rules than $L_0$-Aleph-induce).

%With $L_1$-Tilde (Fig. \ref {curves_1}, curve(a)), we observed a clear accuracy improvement over both $L_0$-Tilde (Fig. APPENDIX REFERENCE) and $L_0$-Aleph-induce (Fig. \ref {curves_1} curve (b)). We note, however, that the bridge experts found the $L_1$-Tilde trees more difficult to read than the rule-based output produced by $L_0$-Aleph-induce. $L_1$-Aleph-induce gave results similar to those of $L_0$-Aleph-induce.

Following these experiments, we had bridge experts do a thorough analysis of one of the successful $L_1$-Tilde outputs. Their goal was to create a sub-model which was much easier to interpret than the large decision trees\footnotemark, and had an accuracy comparable to that seen by $L_1$-Tilde. We also used the experts' insights to further revise the domain theory, in the hope of learning a simpler model with Aleph and Tilde. %After investigating  and post-processing one of the decision tree output by $L_2$-Tilde we could  however manually build a logic program with good precision that Aleph could have discovered, through some modification in its configuration. We have therefore modified Aleph's language bias  and turned its search strategy to induce\_Max in order to learn new models (curve (c) in Fig. \ref {curves_1}) deemed satisfactory by experts in the field and with performances similar to Tilde. 
We describe this process in the next section.
\footnotetext{The experts noted that, in general, the Tilde trees were more difficult to read than the rule-based output produced by Aleph.}
%\begin{figure}


%\begin{figure}
%\centering
%\begin{tabular}{c}
%\includegraphics[width=0.7\textwidth]{plot/aleph_max_acc.png}
%\end{tabular}
%\caption{Courbes de precision, moyennées sur 50 runs pour Aleph, avec la stratégie induce\_max}
%\label{curves_2}
%\end{figure}

\begin {figure}
\begin {center}
\begin {tabular} {cc}
\includegraphics [width = 0.5 \textwidth] {plot/accuracy_1.png}
&
\includegraphics [width = 0.5 \textwidth] {plot/accuracy_2.png}
\end {tabular}
\end {center}
\caption {Average model accuracy}
\label {accuracy_chart}
\end {figure}

\begin {figure}
\begin {center}
\begin {tabular} {cc}
\includegraphics [width = 0.5 \textwidth] {plot/complexity_aleph.png}
&
\includegraphics [width = 0.5 \textwidth] {plot/complexity_tilde.png}
\end {tabular}
\end {center}
\caption {Average model complexity}
\label {complexity_chart}
\end {figure}

\section {Expert Rule Analysis and new Experiments}
\label {analyse}
To find an $L_1$-Tilde output tree for the experts to analyse, we chose a model with good accuracy and low complexity (a large tree would be too hard to parse for a bridge expert). A subtree of the chosen $L_1$-Tilde output is displayed in Listing \ref{best-tree-tilde} (the full tree is displayed in Listing \ref{best-tree-tilde-complete} in the Appendix). Despite the low complexity of this tree (only 15 nodes), it remains somewhat difficult to interpret.


\noindent
\begin{minipage}{\linewidth}
{\footnotesize
 \begin{lstlisting}[frame = single, caption = Part of a tree learned by Tilde, label = best-tree-tilde]
decision(-A,-B,-C,-D,-E)
nb(A,-F,-G),gteq(G,6) ? 
+--yes: hcp(A,4) ? 
|       +--yes: [pass]
|       +--no:  [bid]
+--no:  hcp(A,-H),gteq(H,16) ? 
        +--yes: [bid]
        +--no:  nb(A,spade,-I),gteq(I,1) ? 
                +--yes: lteq(I,1) ? 
                |       +--yes: hcp(A,-J),lteq(J,5) ? 
                |       |       +--yes: [pass]
                |       |       +--no:  nb(A,-K,5) ? 
                |       |               +--yes: hcp(A,6) ? 
                |       |               |       +--yes: [pass]
                |       |               |       +--no:  [bid]
                |       |               +--no:  [pass]
\end{lstlisting}
}
\end{minipage}
%}
%\end{landscape}
%decision(-A,-B,-C,-D,-E)
%nb(A,-F,-G),gteq(G,6) ? 
%+--yes: hcp(A,4) ? 
%|       +--yes: [pass] 2.0 [[bid:0.0,pass:2.0]]
%|       +--no:  [bid] 57.0 [[bid:51.0,pass:6.0]]
%+--no:  hcp(A,-H),gteq(H,16) ? 
%        +--yes: [bid] 6.0 [[bid:6.0,pass:0.0]]
%        +--no:  nb(A,spade,-I),gteq(I,1) ? 
%                +--yes: lteq(I,1) ? 
%                |       +--yes: hcp(A,-J),lteq(J,5) ? 
%                |       |       +--yes: [pass] 11.0 [[bid:0.0,pass:11.0]]
%                |       |       +--no:  nb(A,-K,5) ? 
%                |       |               +--yes: hcp(A,6) ? 
%                |       |               |       +--yes: [pass] 3.0 [[bid:1.0,pass:2.0]]
%                |       |               |       +--no:  [bid] 27.0 [[bid:24.0,pass:3.0]]
%                |       |               +--no:  [pass] 3.0 [[bid:0.0,pass:3.0]]
%                |       +--no:  hcp(A,15) ? 
%                |               +--yes: [bid] 3.0 [[bid:2.0,pass:1.0]]
%                |               +--no:  nb(A,-L,3) ? 
%                |                       +--yes: [pass] 146.0 [[bid:3.0,pass:143.0]]
%                |                       +--no:  hcp(A,11) ? 
%                |                               +--yes: [bid] 3.0 [[bid:3.0,pass:0.0]]
%                |                               +--no:  hcp(A,-M),lteq(M,6) ? 
%                |                                       +--yes: [pass] 15.0 [[bid:0.0,pass:15.0]]
%                |                                       +--no:  lteq(I,2) ? 
    
%, especially for industries where multiple tests have failed.
Simply translating the tree to a decision list does not solve the issue of interpretability. Thus, with the help of bridge experts, we proceeded to do a manual extraction of rules from the given tree, following these post-processing steps:
\begin {enumerate}
\item Natural language translation from relational representations.%, handling of interval negations.
\item 
Removal of nodes with weak support (e.g. a node which tests for precise values of HCP instead of a range).
\item Selection of rules concluding on a $ bid $ leaf.
% (as in line 22 of the listing \ref {best-tree-tilde}).
\item Reformulation of intervals (e.g. combining overlapping ranges of HCP or number of cards).
\item Highlighting the specific number of cards in \Ss {}, and specific $nmpq$ distributions.
\end {enumerate}

The set of rules resulting from this  post-processing, shown in Listing \ref{best-rules-jp}, are much more readable than $L_1$-Tilde trees. Despite it's low complexity, this set of rules has an accuracy of $90.6\%$ on the whole of $S$\footnotemark.

\footnotetext{This number is likely a small overestimate of the model's performance on new data, as these rules were selected by analysing a model that was trained on a subset of $S$}
%Afin de permettre à Aleph d'apprendre un ensemble de règles sur ce vocabulaire,
\noindent
\begin{minipage}{\linewidth}
{\footnotesize 
\begin{lstlisting}[frame = single, caption = Rules extracted from Tilde's best tree, label = best-rules-jp, escapechar = \%]
We bid: 
- With 6+ cards in a non-spade suit or 16+HCP.
- With 0%\Ss{}%.
- With 1%\Ss{}% if 5-4-3-1%\Ss{}% or 5-5-2-1%\Ss{}% in the interval 6-15HCP.
- With 2%\Ss{}% if 5-5-2%\Ss{}%-1 in the interval 7-15HCP.
- With 2%\Ss{}% if 5-4-2-2%\Ss{}% in the interval 11-15HCP.
\end{lstlisting}
}
\end{minipage}

Following this expert review, we created the new $L_2$ language, which only used the predicates that appear in the post-processed rules above. This meant the reintroduction of the \emph{distribution} predicate, the addition of the \emph{nbs} predicate (which is similar to \emph{nb} but denotes only the number of \Ss{} in the hand), and the omission of several other predicates.

%For instance, we removed the $minor$ and $major$ predicates,  which each represents pairs of suits ($minor=\Ds{}\text{ or }\Cs{}$, $major=\Ss{}\text{ or }\Hs{}$), as well as  predicates related to \emph{balanced}, \emph{semi-balanced} or \emph{unbalanced} hands, which are abstractions of the \emph{distribution} predicate.

Using $L_2$ with Aleph-induce results in a much simpler model than $L_1$-Aleph-induce ($6$ rules compared to $16$ when trained on 810 examples), at the cost of somewhat lower accuracy ($83.5\%$ compared to $85.6\%$). The complexity of $L_2$-Tilde was also smaller than it's counterpart $L_1$-Tilde (12 nodes compared to 15), also at the expense of accuracy ($87.3\%$ compared to $89.8\%$). In both cases, the abstracted and simplified $L_2$ language produced models which were far less complex (and thus more easily interpretable), but had a slight degradation in accuracy, when compared with $L_1$.

%We noticed that some of the $L_2$-Aleph-induce rules were equivalent to those in the post-processed Tilde subtree, so we thought that it may be possible to create more concise outputs with a better search of the model space.
%We decided to use Aleph's \emph{induce\_max} strategy instead of \emph{induce}: the search strategy  \emph{induce\_max}  has a higher time cost and can produce rules with large overlaps in coverage, but can generalize better due to the fact that it saturates every example in the training set, not just a subset based on the coverage of a single seed example.

For $L_2$, the more expensive induce\_max search strategy proved useful, with $L_2$-Aleph-induce\_max showing an accuracy of $88.2\%$, second only to $L_1$-Tilde ($89.8\%$). This was at the cost of complexity, with $L_2$-Aleph-induce\_max models having an average of 20 rules compared to 6 for $L_2$-Aleph-induce.

We display in Listing \ref{best-rules-aleph} the first 6 (of 13) rules learned by an $L_2$-Aleph-induce\_max model (see Listing \ref{complete-best-rules-aleph} in the Appendix for the complete set of rules). The rules of this model are relatively easy to apprehend, and the model achieves an accuracy of $89.7\%$ on the whole of $S$.

\noindent
\begin{minipage}{\linewidth}
{\footnotesize 
\begin{lstlisting} [frame=single,caption=First 6 rules of an $L_2$-Aleph-induce\_max model,  label=best-rules-aleph,escapechar=\%]
decision(A,4,B,C,bid) :-
   nbs(A,0).
decision(A,4,B,C,bid) :-
   hcp(A,D), gteq(D,5), nb(A,E,F), gteq(F,6), nbs(A,1).
decision(A,4,B,C,bid) :-
   hcp(A,D), gteq(D,9), nbs(A,1).
decision(A,4,B,C,bid) :-
   hcp(A,D), gteq(D,8), nb(A,E,F), gteq(F,5), nbs(A,1).
decision(A,4,B,C,bid) :-
   hcp(A,D), gteq(D,4), distribution(A,[6,4,2,1]).
decision(A,4,B,C,bid) :-
   hcp(A,D), gteq(D,8), nb(A,E,F), gteq(F,6), nbs(A,2).
\end{lstlisting}
}
\end{minipage}

\begin {table}[hbt!]

\begin {center}
\begin {tabular} {c}
\includegraphics [width = \textwidth] {plot/summary_table.png}
\end {tabular}
\end {center}
\caption {Average accuracy and complexity for all models when trained on 310 and 810 examples, and time taken for training as measure by core hours}
\label {summary_table}
\end {table}

%Quel que soit le nombre de pique :
%       couleur 6+
%    ou HCP >= 14 couleur 2-
%   (ou HCP = 11 et 5422)

%0 pique tout le temps:

%1 pique si :
%      HCP >= 9
%   ou HCP >= 7 et couleur 5+

%2 piques si :
%   couleur <= 1
   %HCP >= 13 et couleur 5+
%Les modèles Tilde donnent de meilleurs résultats sont appris plus efficacement que ceux appris par Aleph. Les experts ont quand même préféré reformuler les modèles de Tilde en ensembles de règles indépendantes les unes des autres, même si cette traduction se fait au prix d'une perte de précision. Cela semble indiquer que bien que les arbres de décisions relationnels soient explicables, ils ne semblent pas être en eux même une explication ou un modèle facilement partageable.
